Causal Discovery from Subsampled Time Series with Proxy Variables

Inferring causal structures from time series data is the central interest of many scientific inquiries. A major barrier to such inference is the problem of subsampling, i.e., the frequency of measurement is much lower than that of causal influence. To overcome this problem, numerous methods have been proposed, yet either was limited to the linear case or failed to achieve identifiability. In this paper, we propose a constraint-based algorithm that can identify the entire causal structure from subsampled time series, without any parametric constraint. Our observation is that the challenge of subsampling arises mainly from hidden variables at the unobserved time steps. Meanwhile, every hidden variable has an observed proxy, which is essentially itself at some observable time in the future, benefiting from the temporal structure. Based on these, we can leverage the proxies to remove the bias induced by the hidden variables and hence achieve identifiability. Following this intuition, we propose a proxy-based causal discovery algorithm. Our algorithm is nonparametric and can achieve full causal identification. Theoretical advantages are reflected in synthetic and real-world experiments.

==> nips23_apppara/algorithm.tex <==
\section{Algorithm}

In this section, we introduce the algorithm to recover the summary DAG, given data observed at $t=1,k+1,...,(\lfloor\frac{T}{k}\rfloor-1)k+1$. The Alg.~\ref{alg:iden sdag} first recovers the MAG according to Prop.~\ref{prop.iden mag}. Then, it connects the recovered MAG to the summary DAG with Prop.~\ref{prop.sdag and mag}. Finally, the summary DAG is identified by Thm.~\ref{thm.iden sdag}.

We first introduce the \emph{Partially Determined Directed Acyclic Graph} (PD-DAG), which will be used to represent the intermediate results of the algorithm. 

\begin{definition}[Partially determined DAG]
A PC-DAG is a DAG with two kinds of directed edges: solid ($\to$) and dashed ($\dashrightarrow$). A solid edge represents a determined causal relation, while a dashed one means the causal relation is still uncertain. We use a meta-symbol, asterisk ($\starto$), to denote any of the two edges. In a PD-DAG $G=(\mathbf{V},\mathbf{E})$, the vertex $A$ is the parent of the vertex $B$ if the edge $A \starto B \in \mathbf{E}$. The definition of \emph{directed path} and \emph{confounding structure} are the same as in DAG.
\end{definition}

\begin{algorithm}
\caption{Identify the summary DAG}
\setstretch{1.2}
\label{alg:iden sdag}
\KwData{Data observed at $t=1,k+1,...,(\lfloor\frac{T}{k}\rfloor-1)k+1$}
\KwResult{The summary DAG}
Construct the skeleton of the MAG with \cite{spirtes2000causation}, orient edges according to Prop.~\ref{prop.iden mag};

For every vertex pair $A,B$, set $A\starto B$ if there are $A(t)\to B(t+k)$ and $A(t+k)\leftrightarrow B(t+k)$ in the MAG. Called the resulted PD-DAG $G_0$;

Set $G=G_0$ and iteratively execute:
\begin{enumerate}[label=(\alph*)]
    \item For every $A\starto B$, check
    \begin{enumerate}[label=(\roman*)]
        \item a directed path from $A$ to $B$ of length $l\leq k-2$;
        \item a directed path from $A$ to $B$ of length $l\leq k-1$ and a confounding structure between $A$ and $B$ of length $(r\leq k-2, q\leq k-2)$;
    \end{enumerate}
    
    If $\exists\,$ (i) or (ii), pass. Otherwise, set $A\to B$ \Comment*[r]{Prop.~\ref{prop.sdag and mag}}

    \item Randomly pick a dashed edge $A\starto B$, check whether $A(t)\ind B(t+k) | \mathbf{Z}(t+1), \mathbf{S}(t)$;

    If independence, remove $A\starto B$. Otherwise, set $A\to B$ \Comment*[r]{Thm.~\ref{thm.iden sdag}}
\end{enumerate}

until all edges in $G$ are solid ones;

\Return $G$
\end{algorithm}








==> nips23_apppara/def_and_asm.tex <==
\section{Problem setup}

Let $\mathbf{X}(t):=\left[X_1(t),...,X_d(t)\right]$ be a multivariate time series with $d$ variables defined at discrete time steps $t=1,...,T$. We assume the data is generated by a first-order structural vector autoregression (SVAR) process:
\begin{equation}
    X_i(t) = f_i(\mathbf{PA}_i(t-1),N_i),
\label{eq.svar model}
\end{equation}
where $f_i$ is the structural function, $\mathbf{PA}_i$ is the parent of $X_i$, and $N_i$ is the exogenous noise.

Eq.~\ref{eq.svar model} assumes that the cause always precedes the effect. It also assumes that the causal mechanism $f_i$ and parents $\mathbf{PA}_i$ are invariant to time. 

We also make the following assumptions.

% note that we change the definition of k:
% o # # # # # o
% <--k_new-->
%   <-k_old->
\begin{assumption}[Semi-causal sufficiency]
We assume that there is an observation every $k$ steps. That is, we can only observe $\mathbf{X}(1),\mathbf{X}(k+1),...,\mathbf{X}((\lfloor\frac{T}{k}\rfloor-1)k+1), k\geq 2$.
\label{asm.subsample}
\end{assumption}

\begin{assumption}[Self causation]
We assume that $X_i \in \mathbf{PA}_i$.
\label{asm.self cause}
\end{assumption}

Causal relations entailed in Eq.~\ref{eq.svar model} can be represented by causal graphs. We first introduce the \emph{full time Directed Acylic Graph (DAG)}, which provides a complete description of the dynamics in the system.

\begin{definition}[Full time DAG]
Let $G:=(\mathbf{V},\mathbf{E})$ be the associated full time DAG of a SVAR process. The vertex set $\mathbf{V}=\{\mathbf{X}(t)\}_{t=1}^T$. The edge set $\mathbf{E}$ contains $X_i(t-1) \to X_j(t)$ if $X_i\in \mathbf{PA}_j$.
\end{definition}

We assume the full time DAG is Markovian and faithful to the joint distribution $\mathbb{P}(\mathbf{X}(1),...,\mathbf{X}(T))$.

\begin{assumption}[Markovian and faithfulness]
For disjoint vertex sets $\mathbf{A},\mathbf{B},\mathbf{Z} \subseteq \mathbf{V}$, $\mathbf{A} \ind_G \mathbf{B} | \mathbf{Z} $ if and only if $\mathbf{A} \ind \mathbf{B} | \mathbf{Z}$.
\label{asm.mark and faith}
\end{assumption}

In practice, it is often sufficient to know the causal relations between time series as a whole, without knowing precisely the relations between time instants. In this regard, one can summarize the causal relations with the \emph{summary DAG}.

\begin{definition}[Summary DAG]
Let $G:=(\mathbf{V},\mathbf{E})$ be the associated summary DAG of a SVAR process. The vertex set $\mathbf{V}=\mathbf{X}$. The edge set $\mathbf{E}$ contains $X_i \to X_j (i \neq j)$ if $X_i \in \mathbf{PA}_j$.
\end{definition}

Our goal is to recover the summary DAG, given data observed at $t=1,k+1,...,(\lfloor \frac{T}{k}\rfloor)k+1$.

==> nips23_apppara/identifiability_v1.tex <==
\section{Identifiability}
\label{sec.app identify}

We first show that the MAG over the observed variables $\mathbf{X}(t)$, for $t=1,k+1,...,(\lfloor\frac{T}{k}\rfloor-1)k+1$, is identifiable from the observation data.

\begin{proposition}[Identifiability of the MAG]
Suppose that (\ref{eq.svar model}), Asm.~\ref{asm.subsample}, and Asm.~\ref{asm.mark and faith} hold, then the MAG over $\mathbf{X}(t)$, for $t=1,k+1,...,(\lfloor\frac{T}{k}\rfloor-1)k+1$, is identifiable, \emph{i.e.}, the skeleton and edge orientations can be uniquely decided from the joint distribution $\mathbb{P}(\mathbf{X}(1),\mathbf{X}(k+1),...,\mathbf{X}((\lfloor\frac{T}{k}\rfloor-1)k+1))$.
\label{prop.iden mag}
\end{proposition}

To prove Prop.~\ref{prop.iden mag}, we first introduce the following lemma, which studies the property of the path between a vertex at $t$ and a vertex at $t+\tau$ ($\tau \geq 0$).

\begin{lemma}
Suppose that there is a path between $A(t),B(t+\tau)$ ($\tau \geq 0$) denoted as $p=A(t),V_1,...,V_r,B(t+\tau)$, if $\exists\, V_i$ on $p$ such that $time(V_i)\geq t+\tau$, then there is a collider on $p$ at $time\geq t+\tau$.
\label{lemma.future path collider}
\end{lemma}

\begin{proof}
We discuss two possible cases and show that $p$ always contains a collider at $time\geq t+\tau$.
\begin{enumerate}[label=\arabic*.,leftmargin=*]
    \item $\forall\, V_i, time(V_i)\leq t+\tau$. In this case, there is a vertex $V_j$ on $p$ such that $time(V_j)=t+\tau$. Consider its adjacent vertices $V_{j-1},V_{j+1}$ on the path. According to our assumption, we have $time(V_{j-1})=time(V_{j+1})=t+\tau-1$. Hence, according to the causal precedence assumption, the edges among $V_{j-1},V_j,V_{j+1}$ are $V_{j-1}(t+\tau-1) \to V_j(t+\tau) \leftarrow V_{j+1}(t+\tau+1)$, which means $V_j(t+\tau)$ is a collider on $p$ at $time=t+\tau$.
    \item $\exists\,V_i, time(V_i)>t+\tau$. Let $j:=\arg\max_{i}time(V_i)$ and $t^*:=time(V_j)$. We have $t^* >t+\tau$. Consider the vertices $V_{j-1},V_j,V_{j+1}$, the edges among them are $V_{j-1}(t^* -1) \to V_j(t^*) \leftarrow V_{j+1}(t^* -1)$. Hence, $V_j(t^*)$ is a collider on $p$ at $time>t+\tau$.
\end{enumerate}
\end{proof}

\newenvironment{proof_prop_iden_mag}{
  \renewcommand{\proofname}{Proof of Prop.~\ref{prop.iden mag}}\proof}{\endproof}

\begin{proof_prop_iden_mag}
According to \citep{spirtes2000causation,zhang2008completeness}, the skeleton of the MAG is identifiable under Asm.~\ref{asm.mark and faith}. 

The orientation of edges in the MAG is either directed ($\to$) or bi-directed ($\leftrightarrow$). Since we assume that the cause must precedes the effect, instantaneous edges\footnote{An edge between $A,B$ is an instantaneous edge if $time(A)=time(B)$.} in the MAG must be bi-directed. In the following, we show that lagged edges in the MAG must be directed and cross $k$ time steps, \emph{e.g.}, $A(t) \to B(t+k)$.

Suppose that $A(t_1)$ and $B(t_2)$ ($t_2>t_1$) are adjacent in the MAG. We first prove that $t_2=t_1+k$. Prove by contradiction. Since $A(t_1)$ and $B(t_2)$ are adjacent in the MAG, there is an inducing path $p=A(t_1),V_1,...,V_r,B(t_2)$ between them in the full time DAG. Suppose that $t_2\neq t_1+k$, in other words, $t_2 \geq t_1+2k$. Since the order of the SVAR process is $1$, there exist $V_i$ on $p$ such that $time(V_i)=t_1+k, time(V_{i+1})=t_1+k+1$. Hence, $V_i(t_1+k)$ is neither latent nor a collider\footnote{$V_i(t_1+k) \to V_{i+1}(t_1+k+1)$ means $V_i(t_1+k)$ can not be a collider.}. As a result, the path $p$ is not an inducing path, which is a contradiction. 

Next, we prove that the edge between $A(t),B(t+k)$ is directed. We prove this by showing that $A(t) \leftrightarrow B(t+k)$ can not be true. Prove by contradiction. Suppose that we have $A(t) \leftrightarrow B(t+k)$ in the MAG, then there is an inducing path $p=A(t),V_1,...,V_r,B(t+k)$ between $A(t),B(t+k)$, and $A(t) \not \in \mathbf{An}(B(t+k))$\footnote{$B(t+k)$ can not be the ancestor of $A(t)$ according to the causal precedence assumption.} in the full time DAG. There are three kinds of possible inducing paths:
\begin{enumerate}[label=\arabic*.]
    \item $\exists\, V_i$ such that $time(V_i)\geq t+k$;
    \item $\forall\, V_i$, $time(V_i)<t+k$ and $time(V_i)>t$;
    \item $\forall\, V_i$, $time(V_i)<t+k$ and $\exists\, V_j$ such that $time(V_j)\leq t$.
\end{enumerate}
In the following, we will show neither of these paths exist, which is a contradiction and shows that the edge between $A(t),B(t+k)$ is directed.
\begin{enumerate}[label=\arabic*.,leftmargin=*]
    \item $\exists\, V_i$ such that $time(V_i)\geq t+k$. In this case, according to Lemma~\ref{lemma.future path collider}, there is a collider on $p$ at $time\geq t+k$. Since the assumed causal precedence, the collider can not be the ancestor of $A(t)$ or $B(t+k+1)$. Hence, the path $p$ is not an inducing path.
    \item $\forall\, V_i$, $time(V_i)<t+k$ and $time(V_i)>t$. In other words, we have $time(V_i)=t+1,..,t+k-1$. We show that in this case, we have $A(t) \in \mathbf{An}(B(t+k))$ in the full time DAG, which contradicts with $A(t) \leftrightarrow B(t+k)$ in the MAG. 
    
    Specifically, when $k=2$, the path is $p=A(t) \to V_1(t+1) \to B(t+2)$. Hence, $A(t) \in \mathbf{An}(B(t+k))$. When $k\geq 3$, consider the first \contour{black}{$\leftarrow$} edge along the path\footnote{If all edges among the path are $\to$, then $A(t) \in \mathbf{An}(B(t+k))$.}, we have $A(t)\doubleto V_{i-1}(t_i+1)$ \contour{black}{$\leftarrow$} $V_i(t_i)$ and $i\geq 3$. Therefore, $V_{i-1}(t_i+1)$ is the descendent of $A(t)$ and a collider on $p$. According to the definition of the inducing path, $V_{i-1}(t_i+1)$ is the ancestor of $B(t+k)$, which means $A(t) \in \mathbf{An}(B(t+k))$.
    \item $\forall\, V_i$, $time(V_i)<t+k$ and $\exists\, V_j$ such that $time(V_j)\leq t$. In this case, we further consider two possibilities,
    \begin{enumerate}[label=\alph*.]
        \item $\forall\,V_i, t\leq time(V_i) < t+k$. In this case, there is a vertex $V_j$ on $p$ such that $time(V_j)=t$ and we have $V_{j-1}(t+1) \leftarrow V_j(t) \to V_{j+1}(t+1)$. Therefore, $V_j(t)$ is neither a latent variable nor a collider, which means $p$ is not an inducing path.
        \item $\forall\, V_i, time(V_i) < t+k$ and $\exists\, V_i$ such that $time(V_i)<t$. In this case, we have $p=A(t),...,V_i(t-\tau),...,B(t+k)$ ($\tau>0$). As a result,there is a vertex $V_j$ on $p$ between $V_i(t-\tau)$ and $B(t+k)$ such that $time(V_j)=t$ and $time(V_{j+1}=t+1$. Therefore, $V_j(t)$ is neither a latent variable nor a collider, which means $p$ is not an inducing path.
    \end{enumerate}
\end{enumerate}
To conclude, we have shown that if there is an inducing path between $A(t),B(t+k)$, then $A(t) \in \mathbf{An}(B(t+k))$, which means all lagged edges in the MAG are directed ones.
\end{proof_prop_iden_mag}

Next, we connect the summary DAG to the MAG with Prop.~\ref{prop.sdag and mag}. For this purpose, we first introduce the some graph structures in the summary DAG.

\begin{definition}[Graph structures]
In the summary DAG,
\begin{enumerate}[label=\arabic*.]
    \item A \emph{directed path} $p_{AB}$ from $A$ to $B$ is a sequence of distinct vertices $A,V_1,...,V_l,B$ ($l\geq 0$\footnote{A directed path of length $l=0$ means $A \to B$.}) such that $A$ is the parent of $V_1$, $V_i$ is the parent of $V_{i-1}$ for $i=2,...,l$, and $V_l$ is the parent of $B$. The length of the directed path is $l$. 
    \item Two directed paths $p_{A B_1}, p_{A B_2}$ (\emph{resp.}) from $A$ to $B_1$ and $B_2$ are called \emph{disjoint} if they do not share any non-startpoint vertex.
    \item A confounding structure $c_{AB}$ of length $(r,q)$ between $A$ and $B$ consists of: a vertex $U$, a directed path $p_{UA}$ from $U$ to $A$ of length $r$, and a directed path $p_{UB}$ from $U$ to $B$ of length $q$, where $p_{UA}$ and $p_{UB}$ are disjoint.
\end{enumerate}
\label{def.confounding struct}
\end{definition}

The following proposition describe the relation between the summary DAG and the MAG.
\begin{proposition}[Summary DAG and MAG]
\,
\begin{enumerate}[label=\arabic*.]
    \item If there is $A\to B$ in the summary DAG, then, there are $A(t) \to B(t+k)$ and $A(t+k) \leftrightarrow B(t+k)$ in the MAG;
    \item If there is $A(t) \to B(t+k)$ in the MAG, then, there is a directed path from $A$ to $B$ of length $l\leq k-1$ in the summary DAG;
    \item If there is $A(t+k)\leftrightarrow B(t+k)$ in the MAG, then, in the summary DAG, at least one of the following structures exists:
    \begin{enumerate}[label=\alph*.]
        \item A directed path\footnote{The path can be from $A$ to $B$ or from $B$ to $A$.} $p$ between $A$ and $B$ of length $l\leq k-2$;
        \item A confounding structure $c$ between $A$ and $B$ of length $(r\leq k-2, q\leq k-2)$.
    \end{enumerate}
\end{enumerate}
Therefore, if there are $A(t) \to B(t+k)$ and $A(t+k) \leftrightarrow B(t+k)$ in the MAG, then, in the summary DAG, at least one of the following structures exists:
\begin{enumerate}[label=\arabic*.]
    \item A directed path $p_{AB}$ from $A$ to $B$ of length $l\leq k-2$;
    \item A directed path $p_{AB}$ from $A$ to $B$ of length $l=k-1$ and a confounding structure $c_{AB}$ between $A$ and $B$ of length $(r\leq k-2,q\leq k-2)$.
\end{enumerate}
\label{prop.sdag and mag}
\end{proposition}

\begin{proof}
\begin{enumerate}[label=\arabic*.,leftmargin=*]
    \item Suppose that there is $A\to B$ in the summary DAG. Then, there is a directed inducing path $p_1=A(t)\to A(t+1)\doubleto A(t+k-1)\to B(t+k)$ from $A(t)$ to $B(t+k)$ in the full time DAG. Thus, we have $A(t) \to B(t+k)$ in the MAG. 
    
    Besides, there is an inducing path $p_2=A(t+k) \leftarrow A(t+k-1) \to B(t+k)$ in the full time DAG, which means we have $A(t+k) \leftrightarrow B(t+k)$ in the MAG.
    \item Suppose that there is $A(t) \to B(t+k)$ in the MAG. Then, there is a directed path $A(t)\to V_1(t+1) \doubleto V_{k-1}(t+k-1) \to B(t+k)$ in the full time DAG. Denote the number of $V_i$ such that $V_i=A$ as $r$, then, we have $0\leq r \leq k-1$. Hence, in the summary DAG, there is a directed path from $A$ to $B$ of length $l=k-r-1$ and we have $0 \leq l \leq k-1$.
    \item Suppose that there is $A(t+k)\leftrightarrow B(t+k)$ in the MAG, we will show that there is a latent confounder $U$ between $A(t+k)$ and $B(t+k)$ such that $t+1\leq time(U)\leq t+k-1$. 
    
    In this regard, if $U=A$ or $U=B$, there is a directed path between $A$ and $B$ of length $l\leq k-2$; Otherwise when $U\neq A$ and $U\neq B$, there is a confounding structure between $A$ and $B$ of length $(r\leq k-2,q\leq k-2)$.

    In the following, we prove that there is a latent confounder $U$ between $A(t+k)$ and $B(t+k)$ such that $t+1\leq time(U)\leq t+k-1$. Prove by contradiction. Suppose that $time(U)\leq t$ or $time(U)\geq t+k$. If $time(U)\leq t$, then on the directed inducing path from $U$ to $A$, there is a vertex at time $t$, which means the path can not be an inducing path. If $time(U)\geq t+k$, then there is a collider on the inducing path between $U$ and $A$ according to Lemma~\ref{lemma.future path collider}, which means the path is not directed and $U$ is not a latent confounder. Hence, the time of the latent confounder $U$ is between $t+1$ and $t+k-1$.
\end{enumerate}
\end{proof}

With Prop.~\ref{prop.iden mag}, Prop.~\ref{prop.sdag and mag}, and the single proxy causal discovery method, we are ready to construct the identifiability of the summary DAG. 

For two vertex $A,B$, let the vertex set $\mathbf{Z}$ contain $A$ and any $Z_i\neq B$ such that $A(t)\to Z_i(t+k)$ in the MAG and $Z_i$ is not $B$'s descendant\footnote{This can be justified from the MAG. Specifically, if $Z_i$ is the descendant of $B$, then there is $B(t) \to V_1(t+k), V_1(t) \to V_2(t+k), ..., V_l(t)\to Z_i(t+k)$ in the MAG.}. Let the vertex set $\mathbf{S}$ contains any $S_i\neq A$ such that $S_i(t) \to B(t+k)$ or $S_i(t) \to Z_j(t+k)$ for some $Z_j \in \mathbf{Z}$ in the MAG.

\begin{theorem}[Identifiability of summary DAG]
Assuming that (\ref{eq.svar model}) and Asm.~\ref{asm.subsample}-\ref{asm.tv-lip} hold, the summary DAG is identifiable for any finite $k\geq 2$. Specifically,
\begin{enumerate}[label=\arabic*.]
    \item There is $A\to B$ in the summary DAG if and only if there are $A(t)\to B(t+k), A(t+k)\leftrightarrow B(t+k)$ in the MAG, and the set $\mathbf{Z}(t+1)\cup \mathbf{S}(t)$ is not sufficient to \emph{d}-separate $A(t),B(t+k)$ in the full time DAG. 
    \item The condition ``the set $\mathbf{Z}(t+1)\cup \mathbf{S}(t)$ is not sufficient to \emph{d}-separate $A(t),B(t+k)$ in the full time DAG'' can be justified by testing whether $A(t) \ind B(t+k) | \mathbf{Z}(t+1)\cup \mathbf{S}(t)$ with proxy variables.
\end{enumerate}
\label{thm.iden sdag}
\end{theorem}

\begin{proof}
\begin{enumerate}[label=\arabic*.,leftmargin=*]
    \item $\Rightarrow$. Suppose that there is $A \to B$ in the summary DAG. According to Prop.~\ref{prop.sdag and mag}, we have $A(t) \to B(t+k)$ and $A(t+k) \leftrightarrow B(t+k)$ in the MAG. In addition, in the full time DAG, there is a directed path $p=A(t)\to B(t+1)\doubleto B(t+k)$ from $A(t)$ to $B(t+k)$, which is not \emph{d}-separated by $\mathbf{Z}(t+1)\cup \mathbf{S}(t)$ (because $B \not \in \mathbf{Z}$).
    
    $\Leftarrow$. Suppose that there are $A(t) \to B(t+k)$ and $A(t+k) \leftrightarrow B(t+k)$ in the MAG. According to Prop.~\ref{prop.sdag and mag}, at least one of the following structures exists:
    \begin{enumerate}[label=\alph*.]
        \item $A\to B$;
        \item A directed path $p_{AB}$ from $A$ to $B$ of length $0<l\leq k-2$;
        \item A directed path $p_{AB}$ from $A$ to $B$ of length $l=k-1$ and a confounding structure $c_{AB}$ between $A$ and $B$ of length $(r\leq k-2,q\leq k-2)$.
    \end{enumerate}
    In the following, we show that if the set $\mathbf{Z}(t+1)\cup \mathbf{S}(t)$ is not sufficient to \emph{d}-separate $A(t),B(t+k)$ in the full time DAG, $A\to B$ must exist in the summary DAG. We prove this by its contrapositive statement, \emph{i.e.}, if $A\to B$ does not exist, the set $\mathbf{Z}(t+1)\cup \mathbf{S}(t)$ is sufficient to \emph{d}-separate $A(t)$ and $B(t+k)$.

    Consider the path between $A(t)$ and $B(t+k)$ in the full time DAG $p=A(t),V_1,...,V_l,B(t+k)$. There are three possible cases:
    \begin{enumerate}[label=\alph*.]
        \item $\exists\, V_i, time(V_i)\geq t+k$;
        \item $\forall\, V_i, time(V_i)<t+k$ and $\exists\, V_j$ such that $time(V_j)\leq t$;
        \item $\forall\, V_i, t<time(V_i)<t+k$.
    \end{enumerate}
    Next, we will show that if $A\to B$ does not exist, the set $\mathbf{Z}(t+1)\cup \mathbf{S}(t)$ can \emph{d}-separate all these three kinds of paths.
    \begin{enumerate}[label=\alph*.]
        \item For the path that $\exists\, V_i, time(V_i)\geq t+k$. According to Lemma~\ref{lemma.future path collider}, there is a collider at $time\geq t+k$. Because the collider and its descendants are not in $\mathbf{Z}(t+1)\cup \mathbf{S}(t)$, the path is \emph{d}-separated.
        \item For the path that $\forall\, V_i, time(V_i)<t+k$ and $\exists\, V_j$ such that $time(V_j)\leq t$. There is a vertex $V_j$ on the path such that $V_j(t)\to V_{j+1}(t+1) \to V_{j+2}(t+2)\to\!\cdots$\footnote{Strictly, when $k=2$, $V_{j+2}$ is $B(t+2)$.} If the path from $V_j(t)$ to $B(t+k)$ is a directed path, we have $V_j\in \mathbf{S}$ and the path is \emph{d}-separated. Otherwise, there is a collider on the path at $time\geq t+2$. Neither the collider nor its descendants are in $\mathbf{Z}(t+1)\cup \mathbf{S}(t)$, the path is also \emph{d}-separated.
        \item For the path that $\forall\, V_i, t<time(V_i)<t+k$. We have $A(t)\to V_1(t+1) \to V_2(t+2) \to\!\cdots$. If the path from $V_1(t+1)$ to $B(t+k)$ is a directed one, $V_1\in \mathbf{Z}$\footnote{$A(t)\to V_1(t+1)$ means we have $A(t) \to V_1(t+k)$ in the MAG. $V_1$ is the ancestor of $B$, so $V_1 \not\in \mathbf{De}(B)$. Hence, $V_i\in \mathbf{Z}$.}. Otherwise, there is a collider on the path at $time\geq t+2$. Neither the collider nor its descendants are in $\mathbf{Z}(t+1)\cup \mathbf{S}(t)$, the path is also \emph{d}-separated.
    \end{enumerate}

    \item In the following, we show that the condition ``the set $\mathbf{Z}(t+1)\cup \mathbf{S}(t)$ is not sufficient to \emph{d}-separate $A(t),B(t+k)$ in the full time DAG'' can be justified by testing $A(t) \ind B(t+k) | \mathbf{Z}(t+1)\cup \mathbf{S}(t)$ with proxy variables.
    \begin{enumerate}[label=\alph*.]
        \item We first explain that $A(t),B(t+k),\mathbf{Z}(t+1),\mathbf{Z}(t+k)$ have the causal graph shown in Fig.~\ref{fig.ABZ proxy causal graph}.

        \begin{figure}
            \centering
            \includegraphics[width=.4\textwidth]{nips23_appfig/proxy_causal_graph.pdf}
            \caption{Causal graph among $A(t),B(t+k),\mathbf{Z}(t+1),\mathbf{Z}(t+k)$.}
            \label{fig.ABZ proxy causal graph}
        \end{figure}

        \begin{itemize}
            \item $A(t)\to \mathbf{Z}(t+1)$. By definition $A$ is the ancestor of vertices in $\mathbf{Z}$.
            \item $\mathbf{Z}(t+1) \to \mathbf{Z}(t+k)$. By Asm.~\ref{asm.self cause} the self causation edge always exists.
            \item $\mathbf{Z}(t+1) \to B(t+k)$. By definition $B$ is not the ancestor of any vertex in $\mathbf{Z}$.
            \item $\mathbf{Z}(t+1) \leftrightarrow B(t+1)$. According to Prop.~\ref{prop.iden mag}, the instantaneous edge must be bi-directed.
        \end{itemize}
        Indeed, the directed edge $\mathbf{Z}(t+1) \to B(t+k)$ and the bi-directed edge $\mathbf{Z}(t+k)\leftrightarrow B(t+k)$ may not exist. However, according to the theory of single proxy causal discovery, as long as we have $A(t) \ind \mathbf{Z}(t+k) | \mathbf{Z}(t+1),\mathbf{S}(t)$ (which will be proved in the following), we can test whether $A(t) \to B(t+k)$ with the proxy variable $\mathbf{Z}(t+k)$.
        
        \item We next show that $A(t) \ind \mathbf{Z}(t+k) | \mathbf{Z}(t+1),\mathbf{S}(t)$, \emph{i.e.}, $\mathbf{Z}(t+k)$ can act as a legal proxy variable of $\mathbf{Z}(t+1)$. We prove this by showing that all path between $A(t)$ to any $Z_i(t+k)\in \mathbf{Z}(t+k)$ can be \emph{d}-separated by $\mathbf{Z}(t+1)\cup \mathbf{S}(t+1)$. Specifically, we consider two different cases:
        \begin{itemize}
            \item When $A\not \to B$ in the summary DAG. To prove this conclusion, again, consider three kinds of paths $A(t),V_1,...,V_l,Z_i(t+k)$ between $A(t)$ and $Z_i(t+k)$, 
            \begin{enumerate}[label=\roman*.]
                \item For the path that $\exists\, V_i, time(V_i)\geq t+k$. It must contain a collider at $time\geq t+k$. Hence, neither the collider nor its descendant is in $\mathbf{Z}(t+1)\cup\mathbf{S}(t)$ and the path is \emph{d}-separated.
                \item For the path that $\forall\, V_i, time(V_i)<t+k$ and $\exists\, V_j$ such that $time(V_j)\leq t$. Then, there is a vertex $V_j$ on the path such that $V_j(t)\to V_{j+1}(t+1) \to V_{j+2}(t+2)\to\!\cdots$. If the path between $V_j(t)$ and $Z_i(t+k)$ is a directed one, then we have $V_j(t)\in \mathbf{S}(t)$ and the path is \emph{d}-separated. Otherwise, there is a collider on the path between $V_{j+2}(t+2)$ and $Z_i(t+k)$. Thus, neither the collider nor its descendant is in $\mathbf{Z}(t+1)\cup\mathbf{S}(t)$ and the path is also \emph{d}-separated.
                \item For the path that $\forall\, V_i, t<time(V_i)<t+k$. In this case, the path must be $A(t)\to V_1(t+1) \to V_2(t+2) \to\!\cdots$. If the path between $V_1(t1)$ and $Z_i(t+k)$ is a directed one, we have $V_1(t+1)\in \mathbf{Z}(t+1)$, because of the following facts: $V_1\neq B$, $A\to V_1$, $V_1\not\in\mathbf{De}(B)$\footnote{If $V_1\in \mathbf{De}(B)$, since $V_1$ is the ancestor of $Z_i$, we have $Z_i\in \mathbf{De}(B)$, which contradicts with the definition of the vertex set $\mathbf{Z}$.}. As a result, the path is \emph{d}-separated. Otherwise when the path between $V_1(t1)$ and $Z_i(t+k)$ is not a directed one, there is a collider on the path at $time\geq t+2$. Therefore, neither the collider nor its descendant is in $\mathbf{Z}(t+1)\cup\mathbf{S}(t)$ and the path is \emph{d}-separated.
            \end{enumerate}
            \item When $A \to B$ in the summary DAG. In this case, except for the above analysis, we need to extra show that every path $p=A(t)\to B(t+1),V_1,...,V_l,Z_i(t+k)$ can be \emph{d}-separated by $\mathbf{Z}(t+1)\cup \mathbf{S}(t)$. Specifically, since we define $Z_i\not\in\mathbf{De}(B)$, $p$ can not be a directed path. Therefore, starting from $B(t+1)$ along the path, at least one of the edge is $\leftarrow$. As a result, there is a collider on $p$ which is either $B(t+1)$ itself or at $time\geq t+2$. For both cases, neither the collider nor its descendant is in $\mathbf{Z}(t+1)\cup\mathbf{S}(t)$ and the path is \emph{d}-separated.
        \end{itemize}

        

        
    \end{enumerate}
\end{enumerate}    
\end{proof}

==> nips23_apppara/preliminary_v1.tex <==
\section{Preliminary}
\label{sec.app preliminary}
Maximal Ancestral Graph (MAG) is commonly used to represent causal relations among observed variables when subsampling exists. Given any DAG $G$ over $\mathbf{V}=\mathbf{O}\cup \mathbf{L}$, the MAG $M$ over the observed set $\mathbf{O}$ is defined as follows,

\begin{enumerate}[label=\arabic*.,leftmargin=*]
    \item Each pair of variables $A,B \in \mathbf{O}$ are adjacent in $M$ if and only if there is an inducing path\footnote{A path $p$ between $A,B \in \mathbf{O}$ is an \emph{inducing path} relative to $\mathbf{L}$ if every non-endpoint vertex on $p$ is either in $\mathbf{L}$ or a collider, and every collider on $p$ is an ancestor of either $A$ or $B$.} relative to $\mathbf{L}$ between them in $G$.
    \item Edge orientations are decided as follows:
    \begin{enumerate}[label=\alph*.]
        \item $A \to B$ in $M$ if $A \in \mathbf{An}(B)$ in $G$;
        \item $A \leftarrow B$ in $M$ if $B \in \mathbf{An}(A)$ in $G$;
        \item $A \leftrightarrow B$ in $M$ if $A \not\in \mathbf{An}(B)$ and $B \not\in \mathbf{An}(A)$ in $G$.
    \end{enumerate}
\end{enumerate}

In the MAG, the directed edge $A \to B$ means $A$ is the ancestor of $B$. The bi-directed edge $A \leftrightarrow B$ means there is a latent confounder $U$ between $A$ and $B$. 


Specifically, $A \leftrightarrow B$ means there is an inducing path $p$ relative to $\mathbf{L}$ between $A$ and $B$. Since $A \not \in \mathbf{An}(B)$ and $B \not \in \mathbf{An}(A)$, the inducing path $p$ must contains non-mediators, \emph{i.e.}, colliders or confounders. Suppose that there are $r$ confounders on $p$, since between every two confounders there is a collider, the number of colliders on $p$ is $r-1$. Denote the confounders on $p$ as $U_1,...,U_r$, the colliders as $C_1,...,C_{r-1}$, we have $p = A \doubleleftarrows U_1 \doubleto C_1 \doubleleftarrows \cdots \doubleto C_{h-1} \doubleleftarrows U_h \doubleto B$. According to the definition of inducing path, each collider $C_i$ on $p$ is the ancestor of either $A$ or $B$. Based on this, the following algorithm is assured to find a latent confounder between $A$ and $B$.


\begin{algorithm}
\caption{Find the latent confounder}
\label{alg:A<->B lat confounder}
\For{$i=1,...,r-1$}{
    \If{$C_i\in \mathbf{An}(B)$}{
        \Return $U_i$ \Comment*[r]{ $A \doubleleftarrows C_{i-1}\doubleleftarrows U_i \doubleto C_i \doubleto B$ }
    }
}
\Return $U_r$ \Comment*[r]{ $A \doubleleftarrows C_{r-1}\doubleleftarrows U_r \doubleto B$ }
\end{algorithm}

When there is a latent mediator $U$ between $A$ and $B$ such that $A\doubleto U \doubleto B$, it is generally not feasible to identify whether $A$ has a directed causal effect on $B$, \emph{i.e.}, $A\to B$. 

The recent progress of \emph{single proxy causal discovery} allows us to identify whether $A \to B$ when a proxy variable $W$ of $U$ is available. To achieve the identifiability, the following smoothness assumption is required:

\begin{assumption}[Smoothness]
For three vertices $A,Z,B\in \mathbf{V}$ such that $A \to Z \to B$ in the full time causal graph, let $\mathbb{P}(B|Z)$, $\mathbb{P}(B|A,Z)$ be (\emph{resp.}) the conditional distribution of $B$ give $Z$ and $(A,Z)$. We assume that $z \mapsto \mathbb{P}(B|Z=z)$, $z \mapsto \mathbb{P}(B|A,Z=z)$ are Lipschitz with respect to the Total Variance (TV) distance.
\label{asm.tv-lip}
\end{assumption}

\begin{remark}
The TV-Lipschitz assumption is satisfied by, for example, the addiction noise model $Z=f(Y)+N$, where $f$ is continuous and differentiable, and $N$ is sampled from the exponential family.
\end{remark}



==> nips23_para/algorithm_mz_v1.tex <==
\section{Discovery algorithm}
\label{sec.alg}

In this section, we introduce Alg.~\ref{alg:iden sdag} to recover the summary DAG based on the identifiability results in Sec.~\ref{sec.identify}. Specifically, given the observed data points, Alg.~\ref{alg:iden sdag} first recovers the MAG according to Prop.~\ref{prop.iden mag}. Then, it uses the necessary condition in Prop.~\ref{prop.sdag and mag} to construct semi-determined edges. Finally, among these semi-determined edges, it uses Thm.~\ref{thm.iden sdag} to identify direct causation and remove the indirect ones.

Next, we first introduce the \emph{Partially Determined Directed Acyclic Graph} (PD-DAG), which will be used to represent the intermediate result of the algorithm. 

\begin{definition}[Partially determined DAG]
A PD-DAG is a DAG with two kinds of directed edges: solid ($\to$) and dashed ($\dashrightarrow$). A solid edge represents a determined causal relation, while a dashed one means the causal relation is still uncertain. We use a meta-symbol, asterisk ($\starto$), to denote any of the two edges. In a PD-DAG $G=(\mathbf{V},\mathbf{E})$, the vertex $A$ is the parent of the vertex $B$ if the edge $A \starto B \in \mathbf{E}$. The definition of \emph{directed path} and \emph{confounding structure} are the same as in DAG.
\end{definition}


\SetKwComment{Comment}{/* }{ */}

\begin{algorithm}[htp]
\caption{Identify the summary DAG}
\setstretch{1.2}
\label{alg:iden sdag}
\KwData{Data observed at $t=1,k+1,...,\lfloor\frac{T}{k}\rfloor k+1$}
\KwResult{The summary DAG}
Construct the skeleton of the MAG with \cite{spirtes2000causation}, orient edges according to Prop.~\ref{prop.iden mag};

For every vertex pair $A,B$, set $A\starto B$ if there are $A(t)\to B(t+k)$ and $A(t+k)\leftrightarrow B(t+k)$ in the MAG. Called the resulted PD-DAG $G_0$ \Comment*[r]{Prop.~\ref{prop.sdag and mag}}

Set $G=G_0$ and iteratively execute:
\begin{enumerate}[label=(\alph*)]
    \item For every $A\starto B$, check
    \begin{enumerate}[label=(\roman*)]
        \item a directed path from $A$ to $B$ of length $l\leq k-2$;
        \item a directed path from $A$ to $B$ of length $l\leq k-1$ and a confounding structure between $A$ and $B$ of length $(r\leq k-2, q\leq k-2)$;
    \end{enumerate}
    
    If $\exists\,$ (i) or (ii), pass. Otherwise, set $A\to B$ \Comment*[r]{Prop.~\ref{prop.sdag and mag}}

    \item Randomly pick a dashed edge $A\starto B$, check whether $A(t)\ind B(t+k) | \mathbf{Z}(t+1), \mathbf{S}(t)$;

    If independence, remove $A\starto B$. Otherwise, set $A\to B$ \Comment*[r]{Thm.~\ref{thm.iden sdag}}
\end{enumerate}

until all edges in $G$ are solid ones;

\Return $G$

\begin{remark}
Alg.~\ref{alg:iden sdag} is readily to generalized to cases where the subsampling factor $k$ is unknown, by skipping the step (a) below line-3.
\end{remark}
\end{algorithm}

==> nips23_para/identifiability_mz_v1.tex <==
\section{Structural identifiability}
\label{sec.identify}

In this section, we establish identifiability of the summary DAG. For this purpose, we connect the observational distribution to the summary DAG with the bridge of maximal ancestral graph. 

To be specific, our analysis consists of three progressive results: Prop.~\ref{prop.iden mag}, Prop.~\ref{prop.sdag and mag}, and Thm.~\ref{thm.iden sdag}. First, in Prop.~\ref{prop.iden mag}, we prove that the MAG can be identified from observational data. Then, in Prop.~\ref{prop.sdag and mag}, we show that the identified MAG \emph{almost uniquely} reflects the structure of summary DAG, in the sense that only edges connecting vertices and their descendants cannot be determined due to latent mediation. Finally, in Thm.~\ref{thm.iden sdag}, we identify these edges and hence the entire summary DAG with the proxy variable approach.

Next, we first introduce Prop.~\ref{prop.iden mag}, which shows that the MAG over the observed variable set $\mathbf{O}:=\{\mathbf{X}(1),...,\mathbf{X}(\lfloor \frac{T}{k} \rfloor k+1)\}$ is identifiable.

\begin{proposition}[Identifiability of the MAG]
Assuming (\ref{eq.svar model}), Asm.~\ref{asm.subsample}, and Asm.~\ref{asm.mark and faith}, the MAG over $\mathbf{O}:=\{\mathbf{X}(1),...,\mathbf{X}(\lfloor \frac{T}{k} \rfloor k+1)\}$ is identifiable, \emph{i.e.}, the skeleton and edge orientations can be uniquely derived from the observed joint distribution $\mathbb{P}(\mathbf{O})$.
\label{prop.iden mag}
\end{proposition}

Since identifiability of MAG's skeleton under faithfulness is a well-known result [\citealp{spirtes1999computation}, Chap.~6], we focus on explaining the edge orientations. As shown in Fig.~\ref{fig.illustration graphs} (c), the MAG contains two types of edges: the instantaneous edge, \emph{e.g.} $A(t_3)\leftrightarrow M(t_3)$, that connects vertices at the same time, and the lagged edge, \emph{e.g.} $A(t_1)\to M(t_3)$, that connects vertices at different time. 

For the instantaneous edge, since we assume cause must precede effect, it can not represents causation but latent confounding, and therefore must be bidirected ($\leftrightarrow$). For example, the edge $A(t_3)\leftrightarrow M(t_3)$ in Fig.~\ref{fig.illustration graphs} (c) is induced by the latent confounder $A(t_3) \leftarrow A(t_2) \to M(t_3)$. For the same reason, the lagged edge must be directed ($\to$) from the past to the future. One should also note that the lagged edge only exists between adjacent observations, \emph{e.g.} $t_1\to t_3, t_3\to t_5$ but not $t_1 \to t_5$. This is because our SVAR model is of first-order and any path between discontinuous observations can not be an inducing path. Please refer to Appx.~\ref{sec.identify} for a detailed proof.

\begin{figure}[tp]
    \centering
    \includegraphics[width=.8\textwidth]{nips23_fig/def_structures.pdf}
    \caption{Illustration of Def.~\ref{def.conf struct}. (a) Directed path from $A$ to $B$ of length $l$. (b) Confounding structure between $A$ and $B$ of length $(r,q)$.}
    \label{fig.graph structs}
\end{figure}

To connect the identified MAG to the summary DAG, we first define the following graph structures:
\begin{definition}[Graph structures]
In the summary DAG,
\begin{enumerate}[label=\arabic*.]
    \item A \emph{directed path} $p_{AB}$ from $A$ to $B$ is a sequence of distinct vertices $A,V_1,...,V_l,B$ such that $A$ is the parent of $V_1$, $V_i$ is the parent of $V_{i-1}$ for $i=2,...,l$, and $V_l$ is the parent of $B$. The length of the directed path is $l$. A directed path of length $l=0$ means $A \to B$.
    \item Two directed paths $p_{A B_1}, p_{A B_2}$ (\emph{resp.}) from $A$ to $B_1$ and $B_2$ are called \emph{disjoint} if they do not share any non-startpoint vertex.
    \item A confounding structure $c_{AB}$ of length $(r,q)$ between $A$ and $B$ consists of: a vertex $U$, a directed path $p_{UA}$ from $U$ to $A$ of length $r$, and a directed path $p_{UB}$ from $U$ to $B$ of length $q$, where $p_{UA}$ and $p_{UB}$ are disjoint.
\end{enumerate}
\label{def.conf struct}
\end{definition}

These structures are further explained in Fig.~\ref{fig.graph structs}. Intuitively, a directed path $p_{AB}$ in the summary DAG means $A$ is the ancestor of $B$. Reflected in the MAG, this means a directed edge $A(t)\to B(t+k)$. Meanwhile, it also induces the latent confounder $A(t+k) \doubleleftarrows A(t+1) \doubleto B(t+k)$ and hence results in a bidirected edge $A(t+k)\leftrightarrow B(t+k)$ in the MAG. On the other hand, the bidirected edge in the MAG may also be induced by $A(t+k) \doubleleftarrows U(t+1) \doubleto B(t+k)$, which means there is a \emph{confounding structure} $A\leftarrow U \to B$ in the summary DAG. 

The above intuitions are summarized into Prop.~\ref{prop.sdag and mag} that connects the MAG to the summary DAG:
\begin{proposition}[MAG to Summary DAG]
\,
\begin{enumerate}[label=\arabic*.]
    \item If there is $A(t) \to B(t+k)$ in the MAG, then, there is a directed path from $A$ to $B$ of length $l\leq k-1$ in the summary DAG;
    \item If there is $A(t+k)\leftrightarrow B(t+k)$ in the MAG, then, in the summary DAG, at least one of the following structures exists:
    \begin{enumerate}[label=\alph*.]
        \item A directed path\footnote{The path can be from $A$ to $B$ or from $B$ to $A$.} $p$ between $A$ and $B$ of length $l\leq k-2$;
        \item A confounding structure $c$ between $A$ and $B$ of length $(r\leq k-2, q\leq k-2)$.
    \end{enumerate}
\end{enumerate}
Therefore, if there are $A(t) \to B(t+k)$ and $A(t+k) \leftrightarrow B(t+k)$ in the MAG, then, in the summary DAG, at least one of the following structures exists:

\quad\quad\,
\begin{enumerate*}[series=tobecont,itemjoin=\quad]
    \item $A \to B$; \item A directed path $p_{AB}$ from $A$ to $B$ of length $1\leq l\leq k-2$;
\end{enumerate*}
\begin{enumerate}[resume=tobecont, ,topsep=0pt, partopsep=0pt]
    \item A directed path $p_{AB}$ from $A$ to $B$ of length $l=k-1$ and a confounding structure $c_{AB}$ between $A$ and $B$ of length $(r\leq k-2,q\leq k-2)$.
\end{enumerate}
\label{prop.sdag and mag}
\end{proposition}

\begin{figure}[tp]
    \centering
    \includegraphics[width=\textwidth]{nips23_fig/sdag_proxy.pdf}
    \caption{Distinguishing direct effect ($A\to B$) from indirect effect ($A\doubleto B$) with proxy variables. Note that though (a) and (b) share the same MAG, only the indirect effect in (b): $A(t_1)\to M(t_2) \to B(t_3)$ can be \emph{d}-separated by $M(t_2)$, \emph{i.e.}, $\mathbb{H}_0: A(t_1) \ind_G B(t_3) | M(t_2)$ only holds for (b). To test $\mathbb{H}_0$, we can use $M(t_3)$ as the proxy variable of $M(t_2)$.}
    \label{fig:sdag proxy}
\end{figure}

The significance of Prop.~\ref{prop.sdag and mag} is the following. On the one hand, it provides a necessary condition for $A\to B$ in the summary DAG, \emph{i.e.}, there are $A(t) \to B(t+k)$ and $A(t+k) \leftrightarrow B(t+k)$ in the MAG. On the other hand, it inspires us that to identify direct causation $A\to B$, we need to differentiate it from the indirect one $A\doubleto B$. 

For this purpose, we propose to use the proxy variable approach. Our idea is briefed below: the indirect effect, unlike the direct one, relies on mediation and therefore can be \emph{d}-separated by the mediator. For example, in Fig.~\ref{fig:sdag proxy} (b), the indirect effect $A(t_1)\to M(t_2) \to B(t_3)$ from $A$ to $B$ can be \emph{d}-separated by the mediator $M(t_2)$. To test the \emph{d}-separation, a major barrier is that the mediator is unobserved and hence can not be (explicitly) conditioned on. Nonetheless, under the self causation Asm.~\ref{asm.self cause}, the unobserved mediator always has an observed proxy, \emph{e.g.}, in Fig.~\ref{fig:sdag proxy}, $M(t_3)$ is the proxy of $M(t_2)$. In this regard, we can test whether $A(t_1)\ind_G B(t_3) | M(t_2)$ with the proxy variable $M(t_3)$ and Thm.~\ref{thm.proxy}.

For the general case, the separation set is a bit more complicated to ensure all paths except the one representing direct effect are \emph{d}-separated. Specifically, for two vertices $A, B$, let the vertex set $\mathbf{M}$ contain $A$ and any $M_i\neq B$ such that $A(t)\to M_i(t+k)$ in the MAG and $M_i$ is not $B$'s descendant\footnote{This can be justified from the MAG. Specifically, if $M_i$ is the descendant of $B$, then there is $B(t) \to V_1(t+k), V_1(t) \to V_2(t+k), ..., V_l(t)\to M_i(t+k)$ in the MAG.}. Let the vertex set $\mathbf{S}$ contains any $S_i\neq A$ such that $S_i(t) \to B(t+k)$ or $S_i(t) \to M_j(t+k)$ for some $M_j \in \mathbf{M}$ in the MAG. We then have the following theorem:

\begin{theorem}[Identifiability of summary DAG]
Assuming that (\ref{eq.svar model}) and Asm.~\ref{asm.subsample}-\ref{asm.tv-lip} hold, the summary DAG is identifiable for any finite $k\geq 2$. Specifically,
\begin{enumerate}[label=\arabic*.]
    \item There is $A\to B$ in the summary DAG if and only if there are $A(t)\to B(t+k), A(t+k)\leftrightarrow B(t+k)$ in the MAG, and the set $\mathbf{M}(t+1)\cup \mathbf{S}(t)$ is \emph{not} sufficient to \emph{d}-separate $A(t),B(t+k)$ in the full time DAG. 
    \item The condition ``the set $\mathbf{M}(t+1)\cup \mathbf{S}(t)$ is not sufficient to \emph{d}-separate $A(t),B(t+k)$ in the full time DAG'' can be justified by testing whether $A(t) \ind_G B(t+k) | \mathbf{M}(t+1)\cup \mathbf{S}(t)$ with proxy variables.
\end{enumerate}
\label{thm.iden sdag}
\end{theorem}

Thm.~\ref{thm.iden sdag} implies that to identify whether $A\to B$ in the summary DAG, we can first check the necessary condition of  ``having $A(t)\to B(t+k)$ and $A(t+k)\leftrightarrow B(t+k)$ in the MAG''. If the condition satisfies, we should further distinguish the direct effect from the indirect one by testing $A(t) \ind_G B(t+k) | \mathbf{M}(t+1)\cup \mathbf{S}(t)$. During the test, since the vertex set $\mathbf{M}(t+1)$ is unobservable, we can use its proxy set $\mathbf{M}(t+k)$. The validity of such proxying, \emph{i.e.}, $A(t) \ind_G \mathbf{M}(t+k) | \mathbf{M}(t+1), \mathbf{S}(t)$ is proved in Sec.~\ref{sec.app identify}

==> nips23_para/introduction_mz_v1.tex <==
\section{Introduction}

Dynamic causal systems are the primary subject of study in many scientific investigations, such as pathology, neuroscience, and economics. One common issue confronted by these sciences is the difficulty of collecting sufficiently refined timescale data. In other words, we can only observed a subsampled sequence of the underlying causal interaction. This issue is particularly prominent in the pathology study of Alzheimer's disease (AD): standard MRI examinations on brain atrophy usually take place every six months \cite{petersen2010alzheimer}, while the underlying disease progression can occur much rapidly \cite{doody2001method,thalhauser2012alzheimer}. This can cause series problem for causal identification, such as missing true interactions \cite{gong2015discovering} and adding spurious ones \cite{hyttinen2016causal}.

To resolve this problem, many attempts have been made but the progress remains limited. Structural identifiability is only known to be achievable in linear data \cite{gong2015discovering,gong2017causal,tank2019identifiability}. As for the nonlinear case, many believed only a small part of the causal information (\emph{i.e.} an equivalence class) can be recovered from subsampled data \cite{danks2013learning,plis2015rate,hyttinen2016causal,malinsky2018causal}.


\begin{figure}[tp]
    \centering
    \includegraphics[width=\textwidth]{nips23_fig/ad_8nodes.pdf}
    \caption{Recovered causal relations in Alzheimer's disease, with (a) our method that explicitly models the subsampling and (b) Dynotears \cite{pamfil2020dynotears} that neglects subsampling. Early degenerated regions (Hippocampus, Amygdala, and Temporal) are marked red. Full results are shown in Fig.~\ref{fig.ad_90nodes}.}
    \label{fig.ad_8nodes}
\end{figure}


In this paper, we propose a constraint-based algorithm than can recover the entire causal structure from subsampled time series, without requiring any parametric assumption. Our departure here is that subsampling prevents identifiability mainly because of the hidden variables at the unobserved time steps. Since these variable can not be (explicitly) conditioned on, they can mislead the differentiation of causation from spurious correlation. Therefore, to achieve identifiability, we can use the observed descendant of the hidden variable as its proxy and (implicitly) adjust for its bias, according to the recent proximal causal discovery approach \cite{miao2018identifying,liu2023causal}. Compared with other approaches dealing with hidden variables, the proxy method particularly suits our temporal setting, in the sense that \emph{self causation} \cite{bartlett1946theoretical} (variable at present is generated by its past, also known as \emph{auto-correlation} in time series statistics) provides an excellent choice of proxy variable. 

As for the technical points, we first construct a Maximal Ancestral Graph \cite{spirtes2000causation} (MAG) over the observed variables to represent the ancestral causal information, which contains both (direct) causation and latent-mediator induced spurious correlation. Then, to distinguish causation from correlation, we (implicitly) condition on the latent mediators via their observed proxies. Our method is essentially non-parametric. It only relies on continuity and differentiability of the structural functions in order to conduct valid proximal conditional independence test \cite{liu2023causal}. Our theory is verified by synthetic data and applied to a case study on Alzheimer's disease pathology.

The rest of the paper is organized as follows. First, in Sec.~\ref{sec.preliminary}, we introduce the problem setting, basic assumptions, and background knowledge on MAG and proxy variable; Then, in Sec.~\ref{sec.identify}, we establish theories on structural identifiability. Based on these theories, we introduce the proposed causal discovery algorithm in Sec.~\ref{sec.alg} and verify its effectiveness in Sec.~\ref{sec.exp}. Finally, in Sec.~\ref{sec.conclusion}, we conclude the paper and discuss future works.

==> nips23_para/preliminary_mz_v1.tex <==
\section{Preliminary}
\label{sec.preliminary}

We start by introducing the causal framework and related literature needed to understand our work. They rely on common causality terminology which we review for completeness in Appx.~\ref{sec.app preliminary}.

\noindent\textbf{Time series model.} Let $\mathbf{X}(t):=\left[X_1(t),...,X_d(t)\right]$ be a multivariate time series with $d$ variables defined at discrete time steps $t=1,...,T$. We assume the data is generated by a first-order structural vector autoregression (SVAR) process:
\begin{equation}
    X_i(t) = f_i(\mathbf{PA}_i(t-1),N_i),
\label{eq.svar model}
\end{equation}
where $f_i$ is the structural function, $\mathbf{PA}_i$ is the parent of $X_i$, and $N_i$ is the exogenous noise.

Implicit in (\ref{eq.svar model}) is the assumptions that cause always precedes effect, and that causation is invariant to time, \emph{i.e.}, the causal mechanism $f_i$ and parents $\mathbf{PA}_i$ keeps unchanged across time steps. These assumptions carry the fundamental beliefs of temporal precedence and stability on causality \cite{pearl2009causality}.

Further, to model the subsampling in data generation, we assume:

\begin{assumption}[Weak causal sufficiency]
There is an observation only every $k$ steps. That is, we can only observe $\mathbf{X}(1),\mathbf{X}(k+1),...,\mathbf{X}( \lfloor\frac{T}{k}\rfloor k+1)$ for $k\geq 2$.
\label{asm.subsample}
\end{assumption}
\begin{remark}
    Causal sufficiency \cite{spirtes2000causation} means all variables in the system are observable. Here, what we require is a weaker version of sufficiency, \emph{i.e.}, all variables can be observed at certain time steps.
\end{remark}

Causal relations entailed in (\ref{eq.svar model}) can be represented by causal graphs. We first introduce the \emph{full time Directed Acylic Graph (DAG)}, which provides a complete description of the dynamics in the system.


\begin{definition}[Full time DAG]
Let $G:=(\mathbf{V},\mathbf{E})$ be the associated full time DAG of a SVAR process. The vertex set $\mathbf{V}=\{\mathbf{X}(t)\}_{t=1}^T$. The edge set $\mathbf{E}$ contains $X_i(t-1) \to X_j(t)$ if $X_i\in \mathbf{PA}_j$.
\end{definition}

We assume the full time DAG is Markovian and faithful to the joint distribution $\mathbb{P}(\mathbf{X}(1),...,\mathbf{X}(T))$.

\begin{assumption}[Markovian and faithfulness]
For disjoint vertex sets $\mathbf{A},\mathbf{B},\mathbf{Z} \subseteq \mathbf{V}$, $\mathbf{A} \ind_G \mathbf{B} | \mathbf{Z} $ if and only if $\mathbf{A} \ind \mathbf{B} | \mathbf{Z}$, where $\ind_G$ denotes \emph{d}-separation in $G$ [\citealp{pearl2009causality}, Def.~1.2.3].
\label{asm.mark and faith}
\end{assumption}

In practice, it is often sufficient to know the causal relations between time series as a whole, without knowing precisely the relations between time instants. In this regard, one can summarize the causal relations with the \emph{summary DAG}.

\begin{definition}[Summary DAG]
Let $G:=(\mathbf{V},\mathbf{E})$ be the associated summary DAG of a SVAR process. The vertex set $\mathbf{V}=\mathbf{X}$. The edge set $\mathbf{E}$ contains $X_i \to X_j (i \neq j)$ if $X_i \in \mathbf{PA}_j$.
\end{definition}

In this paper, our goal is to recover the summary DAG, given data observed at $t=1,k+1,...,\lfloor \frac{T}{k}\rfloor k+1$. For this purpose, we need a structure to represent (marginal) causal relations among observed variables and link the full time DAG to the summary DAG. We choose the \emph{Maximal Ancestral Graph (MAG)} [\citealp{zhang2008completeness}, Def.~3], due to its ability to represent causal relations when subsampling exists.

We first introduce the inducing path, which decides the connectivity of MAG. 

\begin{definition}[\citep{zhang2008completeness} Def.~4, Inducing path]
Let $\mathbf{O}$ and $\mathbf{L}$ be (\emph{resp.}) the set of observed and unobserved variables. A path $p$ between $A,B \in \mathbf{O}$ is an inducing path relative to $\mathbf{L}$ if every non-endpoint vertex on $p$ is either in $\mathbf{L}$ or a collider, and every collider on $p$ is an ancestor of either $A$ or $B$.
\label{def.inducing path}
\end{definition}

Given any full time DAG $G$ over $\mathbf{V}$, the corresponding MAG $M_G$ over the observed set $\mathbf{O}:=\{\mathbf{X}(1),...,\mathbf{X}(\lfloor \frac{T}{k} \rfloor k+1)\}$ is defined as follow.

\begin{definition}[Maximal Ancestral Graph]
In $M_G$, two vertices $A,B \in \mathbf{O}$ are adjacent if and only if there is an inducing path relative to $\mathbf{L}:=\mathbf{V}\backslash \mathbf{O}$ between them in $G$. Edge orientation is:
    \begin{enumerate}[label=\arabic*.]
        \item $A \to B$ in $M$ if $A \in \mathbf{An}(B)$ in $G$;
        \item $A \leftarrow B$ in $M$ if $B \in \mathbf{An}(A)$ in $G$;
        \item $A \leftrightarrow B$ in $M$ if $A \not\in \mathbf{An}(B)$ and $B \not\in \mathbf{An}(A)$ in $G$.
    \end{enumerate}
\label{def.mag}
\end{definition}

\begin{remark}
    In the MAG, the directed edge $A \to B$ means $A$ is the ancestor of $B$. The bi-directed edge $A \leftrightarrow B$ means there is an unobserved confounder $U$ between $A$ and $B$. 
\end{remark}

\begin{figure}[tp]
    \centering
    \includegraphics[width=\textwidth]{nips23_fig/illustration_dags.pdf}
    \caption{(a) Summary DAG showing that the causal influence from $A$ to $B$ is mediated by $M$. (b) Full time DAG with subsampling factor $k=2$. Variables at observed time steps ($t_1,t_3,t_5$) are marked gray. (c) MAG over observed variables. The edges $A(t_1)\to M(t_3)$ and $A(t_3)\leftrightarrow M(t_3)$ are (\emph{resp.}) induced by the inducing paths $A(t_1)\to A(t_2)\to M(t_3)$ and $A(t_3) \leftarrow A(t_2) \to M(t_3)$ in the full time DAG. Please refer to the appendix for a detailed explanation.}
    \label{fig.illustration graphs}
\end{figure}

Graph terminologies, including the full time DAG, summary DAG, and MAG, are illustrated in Fig.~\ref{fig.illustration graphs}.

\noindent\textbf{Proximal causal discovery.} Recent works \cite{kuroki2014measurement,miao2018identifying,liu2023causal} find that one can use the descendant (\emph{i.e.} the proxy variable) of an unobserved variable $U$ to differentiate (direct) causation $A\to B$ from latent mediation $A\to U \to B$. Specifically, \citep{liu2023causal} shows that, under mild conditions\footnote{Namely continuity, differentiability of the structural function, and invertibility of the transition matrix. Please refer to Appx.~\ref{sec.app preliminary} for details.}, we have:

\begin{theorem}[\citep{liu2023causal}, Thm.~4.4]
Suppose that there is a valid proxy $W$ of the unobserved mediator $U$ such that $A \ind_G W | U$. Then, under Asm.~\ref{asm.mark and faith}, the null causal hypothesis $\mathbb{H}_0: A \ind_G B |U$ can be tested by checking whether $pr(b|a)\sim pr(w|a)$ has a linear relation.
\label{thm.proxy}
\end{theorem}
\begin{remark}
The null hypothesis means $A$ does not have a direct causal influence on $B$. Hence, any evidence against $\mathbb{H}_0$ is an evidence for (direct) causation $A\to B$. For continuous variables, \citep{liu2023causal} showed that the linear relation $pr(b|a)\sim pr(w|a)$ can be checked with the least square residual of regressing $pr(b|a)$ on $pr(w|a)$, please refer to Appx.~\ref{sec.app preliminary} for details.
\end{remark}

To ensure the existence of proxy variables, we require the following assumption, which asserts the variable $X_i(t)$ is always influenced by its past $X_i(t-1)$.

\begin{assumption}[Self causation]
$X_i \in \mathbf{PA}_i$ for each $i=1,...,d$.
\label{asm.self cause}
\end{assumption}





